Intermittent molecular motion and first passage statistics for the NMR relaxation of confined water

The structure and dynamics of fluids confined in nanoporous media differ from those in bulk, which can be probed using NMR relaxation measurements. We here show, using atomistic molecular dynamics simulations of water in a slit nanopore, that the behavior of the NMR relaxation rate, R1, with varying surface interaction and confinement strength can be estimated from the exchange statistics of fluid molecules between the adsorbed surface layer and the bulk region, where molecules undergo intermittent dynamics. We employ first return passage time calculations to quantify the molecular exchange statistics, thereby linking microscopic parameters of the confined fluid-such as adsorption time, pore size, and diffusion coefficient-to the NMR relaxation rate. This approach allows to predict and interpret the molecular relaxation of fluids at interfaces using merely concepts of statistical mechanics and can be generalized to closed and open geometries.

==> Makefile <==
# Makefile for building the pdf
all: build

# Target to build the PDF
build:
	latexmk -pdf main.tex

# Target to clean up generated files
clean:
	rm -f main.pdf \
	main.aux \
	main.log \
	main.out \
	main.bbl \
	main.blg

